FRIDU: Functional Map Refinement with Guided Image Diffusion

We propose a novel approach for refining a given correspondence map between two shapes. A correspondence map represented as a functional map, namely a change of basis matrix, can be additionally treated as a 2D image. With this perspective, we train an image diffusion model directly in the space of functional maps, enabling it to generate accurate maps conditioned on an inaccurate initial map. The training is done purely in the functional space, and thus is highly efficient. At inference time, we use the pointwise map corresponding to the current functional map as guidance during the diffusion process. The guidance can additionally encourage different functional map objectives, such as orthogonality and commutativity with the Laplace-Beltrami operator. We show that our approach is competitive with state-of-the-art methods of map refinement and that guided diffusion models provide a promising pathway to functional map processing.

==> definitions.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\makeatletter
\DeclareRobustCommand\onedot{\futurelet\@let@token\@onedot}
\def\@onedot{\ifx\@let@token.\else.\null\fi\xspace}

\def\eg{\emph{e.g}\onedot} \def\Eg{\emph{E.g}\onedot}
\def\ie{\emph{i.e}\onedot} \def\Ie{\emph{I.e}\onedot}
\def\cf{\emph{cf}\onedot} \def\Cf{\emph{Cf}\onedot}
\def\etc{\emph{etc}\onedot} \def\vs{\emph{vs}\onedot}
\def\wrt{w.r.t\onedot} \def\dof{d.o.f\onedot}
\def\etal{\emph{et al}\onedot}
\def\ae{a.e.\ }
\def\conf{\emph{cf}\onedot}
\makeatother

\DeclareMathAlphabet\mathbfcal{OMS}{cmsy}{b}{n}

%%%%% Colors
%%% Another Retro %%%
\definecolor{JungleGreen}{RGB}{40, 169, 143}
\definecolor{BatteryChargedBlue}{RGB}{42, 187, 218}
\definecolor{GargoyleGas}{RGB}{250, 213, 66}
\definecolor{LightCarminePink}{RGB}{236, 94, 100}
\definecolor{MaximumPurple}{RGB}{107, 57, 121}


%%%%% Todos
\IfFileExists{todonotes.sty}{%
	\usepackage{todonotes}
	\usepackage{comment}
	\usepackage{setspace}
	\let\todoavailable1	
}{}%

\ifdefined\todoavailable
	\makeatletter
	\newcommand{\inlinetodo}[2][]{%
		\@todo[caption={}, inline, #1]{#2}%
	} 
	\newcommand{\missing}[2][]{ \@todo[color=red!40, #1]{Missing: #2} }
	\newcommand{\addref}{\textcolor{red!40}{\rule{7pt}{7pt}}} % \todo[color=red!40]{Add reference.}
	%	\newcommand{\checkthis}{}
	\newcommand{\checkthis}{\textcolor{red}{$\bullet$}\todo[color=red!40]{Check this.}}
	
	\newcommand{\addfig}{Figure~\textcolor{LightCarminePink}{\rule{7pt}{7pt}} \todo[color=LightCarminePink]{Add figure.}} 
	\newcommand{\Miri}[2][]{\@todo[color=yellow, #1]{Miri: #2}}
	\newcommand{\Martin}[2][]{\@todo[color=yellow, #1]{Martin: #2}}
	\newcommand{\Florine}[2][]{\@todo[color=yellow, #1]{Florine: #2}}
	\newcommand{\Samuel}[2][]{\@todo[color=yellow, #1]{Samuel: #2}}
	\newcommand{\Josua}[2][]{\@todo[color=yellow, #1]{Josua: #2}}
	\makeatother
\else
	\newcommand{\todo}[1]{{\red{TODO: #1}}}
	\newcommand{\missing}[1]{ {\red{missing: [} #1 \red{]!!!}} }
	\newcommand{\addref}{ {\red{Add reference!}} }
	\newcommand{\addfig}{ {\red{Add figure!}} }
	\newcommand{\Miri}[2][]{\red{Miri: [} #2 \red{].}}
	\newcommand{\Martin}[2][]{\red{Martin: [} #2 \red{].}}
	\newcommand{\Florine}[2][]{\red{Florine: [} #2 \red{].}}
	\newcommand{\Samuel}[2][]{\red{Samuel: [} #2 \red{].}}
	\newcommand{\Josua}[2][]{\red{Josua: [} #2 \red{].}}
	\newcommand{\inlinetodo}[2][]{{\red{TODO: {#2} }\hfill\\}}%
\fi

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% math definitions
\newcommand{\R}{\mathbb{R}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\Q}{\mathbb{Q}}
\newcommand{\Z}{\mathbb{Z}}

\newcommand{\id}{\mathrm{id}\,}
\newcommand{\tr}{\mathrm{tr}\,}
\newcommand{\Id}{\mathrm{Id}}
\renewcommand{\bmod}{{\,\mathrm{mod}\,}}
\newcommand{\atan}{{\mathrm{atan}\,}}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
\renewcommand{\d}{\,\mathrm{d}}
\newcommand{\SO}{\mathit{SO}}
\providecommand{\span}{\mathrm{span}}

% objects
\newcommand{\surface}{\mathcal{S}}
\newcommand{\normal}{n}
\newcommand{\sdf}{\phi}
\newcommand{\B}{\mathcal{B}}
\newcommand{\domain}{\Omega}

% objectives
\newcommand{\E}{\mathcal{E}}
\newcommand{\mmloss}{{\E_{\mathrm{MM}}}}
\newcommand{\sdfloss}{{\E_{\mathrm{SDF}}}}
\newcommand{\fitloss}{{\E_{\mathrm{fit}}}}
\newcommand{\normalloss}{{\E_{\normal}}}
\newcommand{\orientloss}{{\E_{\B}}}
